Nuclear matrix elements for neutrinoless double beta decays and spin-dipole giant resonances

Nuclear matrix elements (NMEs) for neutrinoless double beta decays (DBDs) are required for studying neutrino physics beyond the standard model by DBD. The experimental spin-dipole (SD) giant resonance energy and the SD strength are shown for the first time to be closely related to the DBD-NME, and are used for studying the spin-isospin correlation and the quenching of the axial-vector coupling. So they are used to help the theoretical model calculation of the DBD-NME.

==> GIA-HAO/2_gia_formulation.tex <==

\section{Preliminaries}
\subsection{Graph Neural Networks}
Consider a graph $\gG=(A,X)$  with node set $V=\{v_1,v_2,...,v_n\}$ and edge set $E=\{e_1,e_2,...,e_m\}$,
where  $A \in \{0,1\}^{n\times n}$  is the adjacency matrix and $X\in \R^{n \times d}$ is the node feature matrix.
We are interested in the semi-supervised node classification task~\citep{deeprobust}. That is, given the set of labels $Y\in \{0,1,..,C-1\}^n$ from $C$ classes,
we can train a graph neural network $f_\theta$ parameterized by $\theta$ on the training (sub)graph $\gG_{\text{train}}$
by minimizing a classification loss $\mathcal{L}_{\text{train}}$ (e.g., cross-entropy).
Then the trained $f_\theta$ can predict the labels of nodes in test graph $\gG_{\text{test}}$.
A GNN typically follows a neighbor aggregation scheme to recursively update the node representations as:
\begin{equation}
	\label{eq:gnn}
	H^{(k)}_u = \sigma(W_k\cdot\rho(\{H^{(k-1)}_v\}| v\in\mathcal{N}(u)\cup\{u\})),
\end{equation}

where $\mathcal{N}(u)$ is the set of neighbors of node $u$, $H^{(0)}_u=X_u, \forall u \in V$, $H^{(k)}_u$ is the hidden representation of node $u$ after the $k$-th aggregation,
$\sigma(\cdot)$ is an activation function, e.g., $\text{ReLU}$, and $\rho(\cdot)$ is an aggregation function over neighbors, e.g., $\text{MEAN}$ or $\text{SUM}$.%~\citep{gcn,sage,sgc,gin}.
\subsection{Graph Adversarial Attack\protect\footnote{
		We leave more details and reasons about the setting used in this work in Appendix~\ref{sec:adv_setting_appdx}.}}
\label{sec:adv_setting}
The goal of graph adversarial attack is to fool a GNN model, $f_{\theta^*}$, trained on a graph $\gG=(A,X)$ by constructing a graph $\gG'=(A',X')$ with limited budgets $\lVert \gG'-\gG\rVert \leq \triangle$. Given a set of victim nodes $V_{\text{c}}\subseteq V$, the graph adversarial attack can be generically formulated as:
\begin{equation}
	\label{eq:gia_obj}
	\min \ \mathcal{L}_{\text{atk}}(f_{\theta^*}(\gG')),
	\ \text{s.t.}\ {\lVert \gG'-\gG\rVert \leq \triangle},
\end{equation}
where $\theta^* =\argmin_{\theta}\mathcal{L}_{\text{train}}(f_{\theta}(\gG_{\text{train}}))$ and $\mathcal{L}_{\text{atk}}$ is usually taken as $-\mathcal{L}_{\text{train}}$.
Following previous works~\citep{nettack,tdgia}, Graph adversarial attacks can be characterized into graph modification attacks and graph injection attacks by their perturbation constraints.

\textbf{Graph Modification Attack (GMA).} GMA generates $\gG'$ by modifying the graph structure $A$ and the node features $X$ of the original graph $\gG$.
Typically the constraints in GMA are to limit the number of perturbations on $A$ and $X$, denoted by $\triangle_A$ and $\triangle_X$, respectively, as:
\begin{equation}
	\label{eq:gma_cons}
	\triangle_A+\triangle_X\leq \triangle\in\sZ, \norm{A'-A}_0 \leq \triangle_A\in \sZ, \norm{X'-X}_\infty \leq \epsilon \in \R,
\end{equation}
where the perturbation on $X$ is bounded by $\epsilon$ via L-p norm, since we are using continuous features.


\textbf{Graph Injection Attack (GIA).} Differently, GIA generates $\gG'$ by injecting a set of malicious nodes $V_{\text{atk}}$ as
$X'=\begin{bmatrix}
		\ X\hfill        \\
		\ X_{\text{atk}} \\
	\end{bmatrix},
	A'=\begin{bmatrix}
		\ A\hfill          & A_{\text{atk}} \\
		\ A_{\text{atk}}^T & O_{\text{atk}} \\
	\end{bmatrix},
$
where $X_{\text{atk}}$ is the features of the injected nodes, $O_{\text{atk}}$ is the adjacency matrix among injected nodes, and $A_{\text{atk}}$ is the adjacency matrix between the injected nodes and the original nodes. Let $d_u$ denote the degree of node $u$, the constraints in GIA are:
\begin{equation}
	\label{eq:gia_cons}
	|V_{\text{atk}}| \leq \triangle\in\sZ, \ 1\leq d_u\leq b\in\sZ,
	X_{u} \in \mathcal{D}_X \subseteq \R^d,
	\forall u\in V_{\text{atk}},
\end{equation}
where the number and degrees of the injected nodes are limited, $\mathcal{D}_X=\{C\in\R^d,\min(X)\cdot\mathbf{1}\leq C\leq \max(X)\cdot\mathbf{1} \}$ where $\min(X)$ and $\max(X)$ are the minimum and maximum entries in $X$ respectively.

\textbf{Threat Model.}
We adopt a unified setting, i.e., evasion, inductive and black-box, which is also used by Graph Robustness Benchmark~\citep{grb}.
Evasion: The attack only happens at test time, i.e., $\gG_{\text{test}}$, rather than attacking $\gG_{\text{train}}$.
Inductive:  Test nodes are invisible during training.
Black-box: The adversary can not access the architecture or the parameters of the target model.


==> GIA-HAO/3_gia_comparison.tex <==
\section{Power and Pitfalls of Graph Injection Attack}
\label{sec:gia_comparison}
Based on the setting above, we investigate both the advantages and limitations of GIA by comparing it with GMA.
While we find GIA is more harmful than GMA when there is no defense (Theorem~\ref{thm:gia_threat}),
we also find pitfalls in GIA that can make it easily defendable (Theorem~\ref{thm:gia_easy_defend}).

\subsection{Power of Graph Injection Attack}
Following previous works~\citep{nettack}, we use a linearized GNN, i.e., $H^{(k)}=\hat{A}^kX\Theta$, to track the changes brought by attacks.
Firstly we will elaborate the threats of an adversary as follows.% by measuring the optimal value of the objective as Eq.~\ref{eq:gia_obj} that can achieve.

\begin{definition}[Threats]
	\label{def:threats}
	Consider an adversary $\mathcal{A}$, given a perturbation budget $\triangle$,
	the threat of $\mathcal{A}$ to a GNN $f_\theta$ is defined as $\min_{\norm{\gG'-\gG}\leq \triangle}\mathcal{L}_\atk(f_\theta(\gG'))$, i.e., the optimal objective value of Eq.~\ref{eq:gia_obj}.
\end{definition}

With Definition~\ref{def:threats}, we can quantitatively compare the threats of different adversaries.
\begin{theorem}
	\label{thm:gia_threat}
	Given moderate perturbation budgets $\triangle_\gia$ for GIA and $\triangle_\gma$ for GMA, that is,
	let $\triangle_\gia \leq \triangle_\gma \ll |V|\leq |E|$,
	for a fixed linearized GNN $f_\theta$ trained on $\gG$,
	assume that $\gG$ has no isolated nodes,
	and both GIA and GMA follow the optimal strategy,
	then, \mbox{$\forall \triangle_\gma\geq0, \exists \triangle_\gia\leq \triangle_\gma$}, %such that:
	\[
		\mathcal{L}_{\atk}(f_\theta(\gG'_\gia))-\mathcal{L}_{\atk}(f_\theta(\gG'_\gma))\leq 0,
	\]
	where $\gG'_\gia$ and $\gG'_\gma$ are the perturbed graphs generated by GIA and GMA, respectively.
\end{theorem}
We prove Theorem~\ref{thm:gia_threat} in Appendix~\ref{proof:gia_threat}.
Theorem~\ref{thm:gia_threat} implies that GIA can cause more damage than GMA with equal or fewer budgets, which is also verified empirically as shown in Fig.~\ref{fig:motivate_wo_defense}.


Intuitively, the power of GIA mainly comes from its relatively high flexibility in perturbation generation.
Such flexibility enables us to find a mapping that can map any GMA perturbations to GIA perturbations, leading the same influences to the predictions of $f_\theta$.
We will give an example below.
\begin{figure}[t]
	\topspace
	\begin{subfigure}[b]{0.33\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/m2_illustration-2-crop2.pdf}
		\caption{Illustration of $\mathcal{M}_2$ mapping}
		\label{fig:m2_illustration}
	\end{subfigure}
	\begin{subfigure}[b]{0.33\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/m2_vs_gma.pdf}
		\caption{GMA v.s. GIA with $\mathcal{M}_2$}
		\label{fig:gia_vs_gma_mapping}
	\end{subfigure}
	\begin{subfigure}[b]{0.33\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/grb-cora_node_sims_atk_gma_tdgia.pdf}
		\caption{Homophily changes}
		\label{fig:gia_homophily_dist_node_atk}
	\end{subfigure}
	\caption{Power and pitfalls of Graph Injection Attack}
	\label{fig:gia_vs_gma}
	\vspace{-0.1in}
\end{figure}

\begin{definition}[Plural Mapping $\mathcal{M}_2$]
	\label{def:m2_mapping}
	$\mathcal{M}_2$ maps a perturbed graph $\gG'_\gma$ generated by GMA  with only edge addition perturbations,\footnote{We focus on edge addition in later discussions since \cite{advsample_deepinsights} observed that it produces the most harm in GMA. Discussions about the other GMA operations can be found in Appendix~\ref{sec:m2_gma_appdx}.}
	to a GIA perturbed graph $\gG'_\gia=\mathcal{M}_2(\gG'_\gma)$,
	such that:
	\[
		f_\theta(\gG'_\gia)_u=f_\theta(\gG'_\gma)_u,\forall u \in V.
	\]
\end{definition}
As illustrated in Fig.~\ref{fig:m2_illustration}, the procedure of $\mathcal{M}_2$ is,
for each edge $(u,v)$ added by GMA to attack node $u$,
$\mathcal{M}_2$ can inject a new node $w$ to connect $u$ and $v$, and change $X_w$ to make the same effects to the prediction on $u$.
Then GIA can be further optimized to bring more damage to node $u$.
We also empirically verify the above procedure in Fig.~\ref{fig:gia_vs_gma_mapping}. Details about the comparison are in Appendix~\ref{sec:gma_gia_comparison_appdx}.


\subsection{Pitfalls in Graph Injection Attack}

Through $\mathcal{M}_2$, we show that the flexibility in GIA can make it more harmful than GMA when there is no defense,
however, we also find a side-effect raised in the optimization trajectory of $X_w$ from the above example.
Assume GIA uses PGD~\citep{pgd} to optimize $X_w$ iteratively, we find:
\begin{equation}
	\label{eq:gia_lower_sim}
	\text{sim}(X_u,X_w)^{(t+1)} \leq \text{sim}(X_u,X_w)^{(t)},
\end{equation}
where $t$ is the number of optimization steps and $\text{sim}(X_u,X_v)=\frac{X_u\cdot X_v}{\norm{X_u}_2\norm{X_v}_2}$.
We prove the statement in Appendix~\ref{proof:gia_lower_sim}.
It implies that, under the mapping $\mathcal{M}_2$, the similarity between injected nodes and targets continues to decrease as the optimization processes,
and finally becomes lower than that in GMA. We find this is closely related to the loss of \emph{homophily} of the target nodes.

Before that, we will elaborate the definition of homophily in graph adversarial setting.
Different from typical definitions that rely on the label information~\citep{homophily1_birds,homophily2_collective,geom_gcn,beyond_homophily},
as the adversary does not have the access to all labels,
we provide another instantiation of homophily based on node feature similarity as follows:
\begin{definition}[Node-Centric Homophily]
	\label{def:homophily_node}
	The homophily of a node $u$ can be defined with the \mbox{similarity} between the features of node $u$ and the aggregated features of its neighbors:
	\begin{equation}
		\label{eq:homophily_node}
		h_u=\text{sim}(r_u,X_u),\ r_u=\sum_{j \in \mathcal{N}(u)}\frac{1}{\sqrt{d_j}\sqrt{d_u}}X_j,
	\end{equation}
	where $d_u$ is the degree of node $u$ and $\text{sim}(\cdot)$ is a similarity metric, e.g., cosine similarity.
\end{definition}
We also define edge-centric homophily while we will focus primarily on node-centric homophily. Details and reasons are in Appendix~\ref{sec:homophily_edge_appdx}.
With Definition~\ref{def:homophily_node}, combining Eq.~\ref{eq:gia_lower_sim}, we have:
\[
	h_u^\gia \leq h_u^\gma,
\]
where $h_u^\gia$ and $h_u^\gma$ denote the homophily of node $u$ after GIA and GMA attack, respectively.
It implies that GIA will cause more damage to the homophily of the original graph than GMA.
To verify the discovery for more complex cases,
we plot the homophily distributions in Fig.~\ref{fig:gia_homophily_dist_node_atk}.
The blue part denotes the original homophily distribution. Notably, there is an outstanding out-of-distribution (orange) part caused by GIA, compared to the relatively minor (canny) changes caused by GMA.
The same phenomenon also appears in other datasets that can be found in Appendix~\ref{sec:homophily_appdx}.

Having observed the huge homophily damage led by GIA, it is straightforward to devise a defense mechanism aiming to recover the original homophily, which we call \textit{homophily defenders}.
We theoretically elaborate such defenses in the form of edge pruning\footnote{Actually, homophily defenders can have many implementations other than pruning edges as given in Appendix~\ref{sec:more_homo_defender_appdx}, while we will focus on the design above in our discussion.}, adapted from Eq.~\ref{eq:gnn}:
\begin{equation}
	\label{eq:homo_defender}
	H^{(k)}_u = \sigma(W_k\cdot\rho(\{\mathbb{1}_{\text{con}}(u,v)\cdot H^{(k-1)}_v\}| \ v \in\mathcal{N}(u)\cup\{u\}).
\end{equation}
We find that simply pruning the malicious edges identified by a proper condition can empower homophily defenders with strong theoretical robustness against GIA attacks.
\begin{theorem}
	\label{thm:gia_easy_defend}
	Given conditions in Theorem~\ref{thm:gia_threat},
	consider a GIA attack, which \textup{(i)} is mapped by $\mathcal{M}_2$ (Def.~\ref{def:m2_mapping}) from a GMA attack that only performs edge addition perturbations,
	and \textup{(ii)} uses a linearized GNN trained with at least one node from each class in $\gG$ as the surrogate model, and \textup{(iii)} optimizes the malicious node features with PGD.
	Assume that $\gG$ has no isolated node, and has node features as $X_u=\frac{C}{C-1}e_{Y_u}-\frac{1}{C-1}\mathbf{1}\in \R^d$,
	where $Y_u$ is the label of node $u$ and $e_{Y_u}\in\R^d$ is a one-hot vector with the $Y_u$-th entry being $1$ and others being $0$.
	Let the minimum similarity for any pair of nodes connected in $\gG$ be $s_{\gG}=\min_{(u,v)\in E}\text{sim}(X_u,X_v)$ with $\text{sim}(X_u,X_v)=\frac{X_u\cdot X_v}{\norm{X_u}_2\norm{X_v}_2}$.
	For a homophily defender $g_\theta$ that prunes edges $(u,v)$ if $\text{sim}(X_u,X_v)\leq s_{\gG}$,
	we have:
	\[
		\mathcal{L}_{\text{atk}}(g_\theta(\mathcal{M}_2(\gG'_{\text{GMA}})))-\mathcal{L}_{\text{atk}}(g_\theta(\gG'_{\text{GMA}}))\geq 0.
	\]
\end{theorem}
We prove Theorem~\ref{thm:gia_easy_defend} in Appendix~\ref{proof:gia_easy_defend}.
It implies that, by specifying a mild pruning condition, the homophily defender can effectively reduce the harm caused by GIA to be lower than that of GMA.

Considering a more concrete example with $\mathcal{M}_2$,
$X_w$ is generated to make $\mathcal{L}_{\text{atk}}(f_\theta(\mathcal{M}_2(\gG'_{\text{GMA}})))=\mathcal{L}_{\text{atk}}(f_\theta(\gG'_{\text{GMA}}))$ on node $u$ at first.
Then, due to the flexibility in GIA, $X_w$ can be optimized to some $X'_w$ that greatly destroys the homophily of node $u$, i.e., having a negative cosine similarity score with $u$.
Thus, for a graph with relatively high homophily, i.e., $s_{\gG}\geq 0$,
a mild pruning condition such as $\mathbb{1}_{\text{sim}(u,v)\leq 0}(u,v)=0$ could prune all the malicious edges generated by GIA while possibly keeping some of those generated by GMA,
which makes GIA less threatful than GMA.

In the literature, we find that GNNGuard~\citep{gnnguard} serves well for an implementation of homophily defenders as Eq.~\ref{eq:homo_defender}.
With GNNGuard, we verify the strong empirical robustness of homophily defenders against GIA.
As Fig.~\ref{fig:motivate_w_defense} depicts,
when with homophily defenders, GIA can only cause little-to-no damage, while GMA can still effectively perturb the predictions of the target model on some nodes.
To fully demonstrate the power of homophily defenders, we also prove its certified robustness for a concrete GIA case in Appendix~\ref{sec:gia_cer_robo}.


==> GIA-HAO/4-1_gia_unnoticeability.tex <==
\section{Homophily Unnoticeable Graph Injection Attack}
\label{sec:gia_hao}

\subsection{Harmonious Adversarial Objective}
\label{sec:gia_unnoticeability}
As shown in Sec.~\ref{sec:gia_comparison}, the flexibility of GIA makes it powerful
while dramatically hinders its performance when combating against homophily defenders,
because of the great damage to the homophily distribution brought by GIA.
This observation motivates us to introduce the concept of \emph{homophily unnoticeability} that enforces GIA to preserve the original homophily distribution during the attack.
\begin{definition}[Homophily Unnoticeability]
	\label{def:homo_unnoticeable}
	Let the node-centric homophily distribution for a graph $\gG$ be $\mathcal{H}_\gG$.
	Given the upper bound for the allowed homophily distribution shift $\triangle_{\mathcal{H}}\geq 0$,
	an attack $\mathcal{A}$ is homophily unnoticeable if:
	\[
		m(\mathcal{H}_\gG,\mathcal{H}_{\gG'})\leq \triangle_{\mathcal{H}},
	\]
	where $\gG'$ is the perturbed graph generated by $\mathcal{A}$,
	and $m(\cdot)$ is a distribution distance measure.
\end{definition}
Intuitively, homophily unnoticeability can be a supplementary for the unnoticeability in graph adversarial attack that requires a GIA adversary to consider
how likely the new connections between the malicious nodes and target nodes will appear \textit{naturally}.
Otherwise, i.e., unnoticeability is broken, the malicious nodes and edges can be easily detected and removed by database administrators or homophily defenders.
However, homophily unnoticeability can not be trivially implemented as a rigid constraint and be inspected incrementally like that for degree distribution~\citep{nettack}.
For example, a trivial implementation such as clipping all connections that do not satisfy the constraint (Def.~\ref{def:homo_unnoticeable}) will trivially clip all the injected edges due to the unconstrained optimization in GIA.

Considering the strong robustness of homophily defenders, we argue that they can directly serve as external examiners for homophily unnoticeability check.
Satisfying the homophily constraint can be approximately seen as bypassing the homophily defenders.
Obviously, GIA with constraints as Eq.~\ref{eq:gia_cons} can not guarantee homophily unnoticeability,
since it will only optimize towards maximizing the damage by minimizing the homophily of the target nodes.
Hence, we propose a novel realization of the homophily constraint for GIA that enforces it to meet the homophily unnoticeability \textit{softly}.

\begin{definition}[Harmonious Adversarial Objective (HAO)]
	Observing the homophily definition in Eq.~\ref{eq:homophily_node} is differentiable with respect to $X$, we can integrate it into the objective of Eq.~\ref{eq:gia_obj} as:\footnote{Note that we only use HAO to solve for $\gG'$ while still using the original objective to evaluate the threats.}
	\begin{equation}
		\label{eq:gia_obj_harmo}
		\begin{aligned}
			\min _{\lVert \gG'-\gG\rVert \leq \triangle} \ \mathcal{L}^{\text{h}}_{\text{atk}}(f_{\theta^*}(\gG')) & =
			\mathcal{L}_{\text{atk}}(f_{\theta^*}(\gG'))
			-\lambda C(\gG,\gG'),                                                                                      \\
		\end{aligned}
	\end{equation}
	where $C(\gG,\gG')$ is a regularization term based on homophily and $\lambda\geq 0$ is the corresponding weight.
\end{definition}
One possible implementation is to maximize the homophily for each injected node as:
\begin{equation}
	\label{eq:harmo_reg_1}
	C(\gG,\gG') = \frac{1}{|V_{\text{atk}}|}\sum_{u\in V_{\text{atk}}}{h_u}.
\end{equation}
HAO seizes the possibility of
retaining homophily unnoticeability, while still performing effective attacks.
Hence, given the homophily distribution distance measure $m(\cdot)$ in Def.~\ref{def:homo_unnoticeable}, we can infer:
\begin{theorem}
	\label{thm:hao_break_limit}
	Given conditions in Theorem~\ref{thm:gia_easy_defend},
	we have
	$m(\mathcal{H}_\gG,\mathcal{H}_{\gG'_{\text{HAO}}})\!\leq\! m(\mathcal{H}_\gG,\mathcal{H}_{\gG'_{\text{GIA}}})$, hence:
	\[
		\mathcal{L}_{\text{atk}}(g_\theta(\gG'_{\text{HAO}}))-\mathcal{L}_{\text{atk}}(g_\theta(\gG'_{\text{GIA}}))\leq 0,
	\]
	where $\gG'_{\text{HAO}}$ is generated by GIA with HAO, and $\gG'_{\text{GIA}}$ is generated by GIA without HAO.
\end{theorem}
We prove Theorem~\ref{thm:hao_break_limit} in Appendix~\ref{proof:hao_break_limit}.
Intuitively, since GIA with HAO can reduce the damage to homophily,
it is more likely to bypass the homophily defenders, thus being more threatful than GIA without HAO.
We also empirically verify Theorem~\ref{thm:hao_break_limit} for more complex cases in the experiments.


==> GIA-HAO/4-2_gia_algorithm.tex <==
\subsection{Adaptive Injection Strategies}
\label{sec:gia_algorithm}
GIA is generically composed of two procedures, i.e., node injection and feature update, to solve for $\gG'=(A',X')$,
where node injection leverages either the gradient information or heuristics to solve for $A'$, and feature update usually uses PGD~\citep{pgd} to solve for $X'$.
Most previous works separately optimize $A'$ and $X'$ in a greedy manner,
which implicitly assumes that the other will be optimized to maximize the harm.
However, HAO does not follow the assumption but stops the optimization when the homophily is overly broken.
Thus, a more suitable injection strategy for HAO shall \textit{be aware of} retaining the original homophily.
%Thus, previous injection strategies (the optimization procedure of $A_\atk$) may not fully exploit the power of HAO.
To this end, we propose to optimize $A'$ and $X'$ alternatively and introduce three adaptive injection strategies to coordinate with HAO.

\textbf{Gradient-Driven Injection.}
We propose a novel bi-level formulation of HAO to perform the alternative optimization using gradients,
where we separate the optimization of $\gG'=\!(A',X')$ as:
\begin{equation}
  \label{eq:gia_bilevel_obj}
  \begin{aligned}
    X'^*       & =\argmin_{X'\in \Phi(X')}\mathcal{L}_{\text{atk}}(f_{\theta^*}(A'^*,X'))-\lambda_A C(\gG',\gG), \\
    s.t.\ A'^* & = \argmin_{A'\in \Phi(A')}\mathcal{L}_{\text{atk}}(f_{\theta^*}(A',X'))-\lambda_X C(\gG',\gG) , \\
  \end{aligned}
\end{equation}
where $\Phi(A')$ and $\Phi(X')$ are the corresponding feasible regions for $A'$ and $X'$ induced by the original constraints.
Here we use different homophily constraint weights $\lambda_A$ and $\lambda_X$ for the optimizations of $A'$ and $X'$, since $A'$ is discrete while $X'$ is continuous.
We can either adopt Meta-gradients like Metattack~\citep{metattack} (\textbf{MetaGIA}) or directly optimize edge weights to solve for $A'$ (\textbf{AGIA}).
The detailed induction of meta-gradients and algorithms are given in Appendix~\ref{sec:gia_gradient_appdx}.

\textbf{Heuristic-Driven Injection.}
As the state-of-the-art GIA methods are leveraging heuristics to find $A'$, based on TDGIA~\citep{tdgia}, we also propose a variant (\textbf{ATDGIA}) using heuristics as:
\begin{equation}
  \label{eq:tdgia+_score}
  s_u = ((1-p_u)\mathbb{1}(\argmax{(p)}=y'_u))(\frac{0.9}{\sqrt{bd_u}}+\frac{0.1}{d_u}),
\end{equation}
where $s_u$ indicates the vulnerability of node $u$ and $\mathbb{1}(\cdot)$ is to early stop destroying homophily.

\textbf{Sequential Injection} for large graphs. Since gradient methods require huge computation overhead,
we propose a novel divide-and-conquer strategy (\textbf{SeqGIA}) to iteratively select some of the most vulnerable targets with Eq.~\ref{eq:tdgia+_score} to attack.
Detailed algorithm is given in Appendix~\ref{sec:gia_apgd_seq_appdx}.


==> GIA-HAO/5_experiment.tex <==
\section{Experiments}
\label{sec:experiments}


\subsection{Setup \& Baselines}
\label{sec:exp_setups}
\textbf{Datasets.}
We comprehensively evaluate our methods with $38$ defense models on $6$ datasets.
We select two classic citation networks Cora and Citeseer~\citep{cora,citeseer} refined by GRB~\citep{grb}.
We also use Aminer and Reddit~\citep{aminer,sage,saint} from GRB, Arxiv from OGB~\citep{ogb}, and a co-purchasing network Computers~\citep{computers_photo} to cover more domains and scales.
Details are in Appendix~\ref{sec:datasets_appdx}.

\textbf{Comparing with previous attack methods.}
We incorporate HAO into several existing GIA methods as well as our proposed injection strategies to verify its effectiveness and versatility.
First of all, we select \textbf{PGD}~\citep{pgd} as it is one of the most widely used adversarial attacks.
We also select \textbf{TDGIA}~\citep{tdgia} which is the state-of-the-art GIA method.
We adopt the implementations in GRB~\citep{grb} for the above two methods.
We exclude FGSM~\citep{fgsm} and AFGSM \citep{afgsm}, since PGD is better at dealing with non-linear models than FGSM~\citep{pgd}, and AFGSM performs comparably with FGSM but is worse than TDGIA as demonstrated by~\cite{tdgia}.
For GMA methods, we adopt \textbf{Metattack}~\citep{metattack} as one of the bi-level implementations. We exclude Nettack~\citep{nettack} as it is hard to perform incremental updates with GCN (the surrogate model used in our experiments) and leave reinforcement learning methods such as RL-S2V \citep{rls2v} and NIPA \citep{nipa} for future work. More details are given in Appendix~\ref{sec:exp_rl_appdx}.


\textbf{Categories and complexity analysis of attack methods.}
We provide categories and complexity analysis of all attack methods used in our experiments in Table~\ref{tab:complexity}, Appendix~\ref{sec:gia_alg_complexity}.


\textbf{Competing with different defenses.} We select both popular GNNs and robust GNNs as the defense models.
For popular GNNs, we select the three most frequently used baselines, i.e., \textbf{GCN}~\citep{gcn}, \textbf{GraphSage}~\citep{sage}, and \textbf{GAT}~\citep{gat}.
For robust GNNs, we select \textbf{GCNGuard}~\citep{gnnguard} for graph purification approach, and \textbf{RobustGCN}~\citep{robustgcn} for stabilizing hidden representation approach,
as representative ones following the surveys~\citep{sun_gadv_survey,deeprobust}.
Notably, the author-released GCNGuard implementation requires $O(n^2)$ complexity, which is hard to scale up.
To make the comparison fair, following the principle of homophily defenders, we implement two efficient robust alternatives, i.e., Efficient GCNGuard (\textbf{EGuard}) and Robust Graph Attention Network (\textbf{RGAT}).
More details are given in Appendix~\ref{sec:rgat_appdx}.
Besides, we exclude the robust GNNs learning in a transductive manner like ProGNN~\citep{prognn} that can not be adapted in our setting.

\textbf{Competing with extreme robust defenses.}
To make the evaluation for attacks more reliable,
we also adopt two widely used robust tricks Layer Normalization (\textbf{LN})~\citep{layer_norm} and an efficient adversarial training~\citep{fgsm,pgd} method \textbf{FLAG}~\citep{flag}.
Here, as FLAG can effectively enhance the robustness, we exclude other adversarial training methods for efficiency consideration.
More details are given in Appendix~\ref{sec:baseline_detail_appdx}.


\begin{table}[t]
	\topspace
	\caption{Performance of non-targeted attacks against different models}
	\label{tab:eval_non_targeted}
	\resizebox{\textwidth}{!}{
		\scriptsize
		\begin{tabular}{@{}{l}*{13}{c}@{}}
			\toprule
			                                         &              & \multicolumn{3}{c}{{\small Cora ($\downarrow$)}} & \multicolumn{3}{c}{{\small Citeseer($\downarrow$)}} & \multicolumn{3}{c}{{\small Computers($\downarrow$)}} & \multicolumn{3}{c}{{\small Arxiv($\downarrow$)}}                                                                                                                                                                                                                                                                                                          \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
			                                         & HAO          & \multicolumn{1}{c}{\textbf{Homo}}                & \multicolumn{1}{c}{\textbf{Robust}}                 & \multicolumn{1}{c}{\textbf{Combo}}                   & \multicolumn{1}{c}{\textbf{Homo}}                & \multicolumn{1}{c}{\textbf{Robust}} & \multicolumn{1}{c}{\textbf{Combo}} & \multicolumn{1}{c}{\textbf{Homo}} & \multicolumn{1}{c}{\textbf{Robust}} & \multicolumn{1}{c}{\textbf{Combo}} & \multicolumn{1}{c}{\textbf{Homo}} & \multicolumn{1}{c}{\textbf{Robust}} & \multicolumn{1}{c}{\textbf{Combo}} \\ \midrule
			Clean                                    &              & $85.74$                                          & $86.00$                                             & $87.29$                                              & $74.85$                                          & $75.46$                             & $75.87$                            & $93.17$                           & $93.17$                             & $93.32$                            & $70.77$                           & $71.27$                             & $71.40$                            \\  \hdashline[0.5pt/1pt]
			\rule{0pt}{10pt}PGD                      &              & $83.08$                                          & $83.08$                                             & $85.74$                                              & $74.70$                                          & $74.70$                             & $75.19$                            & $84.91$                           & $84.91$                             & $91.41$                            & $68.18$                           & $68.18$                             & $71.11$                            \\
			PGD                                      & $\checkmark$ & $52.60$                                          & $62.60$                                             & $77.99$                                              & $69.05$                                          & $69.05$                             & $73.04$                            & $79.33$                           & $79.33$                             & $87.83$                            & $55.38$                           & $\underline{62.89}$                 & $68.68$                            \\\hdashline[0.5pt/1pt]
			\rule{0pt}{10pt}MetaGIA$^\dagger$        &              & $83.61$                                          & $83.61$                                             & $85.86$                                              & $74.70$                                          & $74.70$                             & $75.15$                            & $84.91$                           & $84.91$                             & $91.41$                            & $68.47$                           & $68.47$                             & $71.09$                            \\
			MetaGIA$^\dagger$                        & $\checkmark$ & $49.25$                                          & $\underline{69.83}$                                 & $76.80$                                              & $68.04$                                          & $68.04$                             & $\underline{71.25}$                & $78.96$                           & $78.96$                             & $90.25$                            & $57.05$                           & $63.30$                             & $69.97$                            \\
			AGIA$^\dagger$                           &              & $83.44$                                          & $83.44$                                             & $85.78$                                              & $74.72$                                          & $74.72$                             & $75.29$                            & $85.21$                           & $85.21$                             & $91.40$                            & $68.07$                           & $68.07$                             & $71.01$                            \\
			AGIA$^\dagger$                           & $\checkmark$ & $\underline{47.24}$                              & $\mathbf{61.59}$                                    & $\mathbf{75.25}$                                     & $70.24$                                          & $70.24$                             & $71.80$                            & $\underline{75.14}$               & $\underline{75.14}$                 & $\underline{86.02}$                & $59.32$                           & $65.62$                             & $69.92$                            \\\hdashline[0.5pt/1pt]
			\rule{0pt}{10pt}TDGIA                    &              & $83.44$                                          & $83.44$                                             & $85.72$                                              & $74.76$                                          & $74.76$                             & $75.26$                            & $88.32$                           & $88.32$                             & $91.40$                            & $64.49$                           & $64.49$                             & $70.97$                            \\
			TDGIA                                    & $\checkmark$ & $56.95$                                          & $73.38$                                             & $79.45$                                              & $\mathbf{60.91}$                                 & $\mathbf{60.91}$                    & $72.51$                            & $\mathbf{74.77}$                  & $\mathbf{74.77}$                    & $90.42$                            & $\underline{49.36}$               & $\mathbf{60.72}$                    & $\mathbf{63.57}$                   \\
			ATDGIA                                   &              & $83.07$                                          & $83.07$                                             & $85.39$                                              & $74.72$                                          & $74.72$                             & $75.12$                            & $86.03$                           & $86.03$                             & $91.41$                            & $66.95$                           & $66.95$                             & $71.02$                            \\
			ATDGIA                                   & $\checkmark$ & $\mathbf{42.18}$                                 & $70.30$                                             & $\underline{76.87}$                                  & $\underline{61.08}$                              & $\underline{61.08}$                 & $\mathbf{71.22}$                   & $80.86$                           & $80.86$                             & $\mathbf{84.60}$                   & $\mathbf{45.59}$                  & $63.30$                             & $\underline{64.31}$                \\\hdashline[0.5pt/1pt]
			\hdashline[0.5pt/3pt]\rule{0pt}{10pt}MLP &              & \multicolumn{3}{c}{{$61.75$}}                    & \multicolumn{3}{c}{{$65.55$}}                       & \multicolumn{3}{c}{{$84.14$}}                        & \multicolumn{3}{c}{{$52.49$}}                                                                                                                                                                                                                                                                                                                             \\ \bottomrule
			\multicolumn{14}{l}{$^\downarrow$The lower number indicates better attack performance.  $^\dagger$Runs with SeqGIA framework on Computers and Arxiv.  }                                                                                                                                                                                                                                                                                                                                                                                                                             \\
		\end{tabular}}
\end{table}



\begin{table}[t]
	\caption{Performance of targeted attacks against different models}
	\label{tab:eval_targeted}
	\resizebox{\textwidth}{!}{
		\scriptsize
		\begin{tabular}{@{}{l}*{13}{c}@{}}
			\toprule
			                                         &              & \multicolumn{3}{c}{{\small Computers($\downarrow$)}} & \multicolumn{3}{c}{{\small Arxiv($\downarrow$)}} & \multicolumn{3}{c}{{\small Aminer($\downarrow$)}} & \multicolumn{3}{c}{{\small Reddit($\downarrow$)}}                                                                                                                                                                                                                                                                                                          \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
			                                         & HAO          & \multicolumn{1}{c}{\textbf{Homo}}                    & \multicolumn{1}{c}{\textbf{Robust}}              & \multicolumn{1}{c}{\textbf{Combo}}                & \multicolumn{1}{c}{\textbf{Homo}}                 & \multicolumn{1}{c}{\textbf{Robust}} & \multicolumn{1}{c}{\textbf{Combo}} & \multicolumn{1}{c}{\textbf{Homo}} & \multicolumn{1}{c}{\textbf{Robust}} & \multicolumn{1}{c}{\textbf{Combo}} & \multicolumn{1}{c}{\textbf{Homo}} & \multicolumn{1}{c}{\textbf{Robust}} & \multicolumn{1}{c}{\textbf{Combo}} \\ \midrule
			Clean                                    &              & $92.68$                                              & $92.68$                                          & $92.83$                                           & $69.41$                                           & $71.59$                             & $72.09$                            & $62.78$                           & $66.71$                             & $66.97$                            & $94.05$                           & $97.15$                             & $97.13$                            \\  \hdashline[0.5pt/1pt]
			\rule{0pt}{10pt}PGD                      &              & $88.13$                                              & $88.13$                                          & $91.56$                                           & $69.19$                                           & $69.19$                             & $71.31$                            & $53.16$                           & $53.16$                             & $56.31$                            & $92.44$                           & $92.44$                             & $93.03$                            \\
			PGD                                      & $\checkmark$ & $71.78$                                              & $71.78$                                          & $85.81$                                           & $\mathbf{36.06}$                                  & $\mathbf{37.22}$                    & $69.38$                            & $34.62$                           & $34.62$                             & $39.47$                            & $\underline{56.44}$               & $\underline{86.12}$                 & $\mathbf{84.94}$                   \\\hdashline[0.5pt/1pt]
			\rule{0pt}{10pt}MetaGIA$^\dagger$        &              & $87.67$                                              & $87.67$                                          & $91.56$                                           & $69.28$                                           & $69.28$                             & $71.22$                            & $48.97$                           & $48.97$                             & $52.35$                            & $92.40$                           & $92.40$                             & $93.97$                            \\
			MetaGIA$^\dagger$                        & $\checkmark$ & $\underline{70.21}$                                  & $\underline{71.61}$                              & $85.83$                                           & $38.44$                                           & $\underline{38.44}$                 & $48.06$                            & $41.12$                           & $41.12$                             & $45.16$                            & $\mathbf{46.75}$                  & $90.06$                             & $90.78$                            \\
			AGIA$^\dagger$                           &              & $87.57$                                              & $87.57$                                          & $91.58$                                           & $66.19$                                           & $66.19$                             & $70.06$                            & $50.50$                           & $50.50$                             & $53.69$                            & $91.62$                           & $91.62$                             & $93.66$                            \\
			AGIA$^\dagger$                           & $\checkmark$ & $\mathbf{69.96}$                                     & $\mathbf{71.58}$                                 & $85.72$                                           & $38.84$                                           & $38.84$                             & $68.97$                            & $35.94$                           & $35.94$                             & $42.66$                            & $80.69$                           & $88.84$                             & $90.44$                            \\\hdashline[0.5pt/1pt]
			\rule{0pt}{10pt}TDGIA                    &              & $87.21$                                              & $87.21$                                          & $91.56$                                           & $63.66$                                           & $63.66$                             & $71.06$                            & $51.34$                           & $51.34$                             & $54.82$                            & $92.19$                           & $92.19$                             & $93.62$                            \\
			TDGIA                                    & $\checkmark$ & $71.39$                                              & $71.62$                                          & $\mathbf{77.15}$                                  & $42.56$                                           & $42.56$                             & $\underline{42.53}$                & $\underline{25.78}$               & $\underline{25.78}$                 & $\underline{29.94}$                & $78.16$                           & $\mathbf{85.06}$                    & $\underline{88.66}$                \\
			ATDGIA                                   &              & $87.85$                                              & $87.85$                                          & $91.56$                                           & $66.12$                                           & $66.12$                             & $71.16$                            & $50.87$                           & $50.87$                             & $53.68$                            & $91.25$                           & $91.25$                             & $93.03$                            \\
			ATDGIA                                   & $\checkmark$ & $72.00$                                              & $72.53$                                          & $\underline{78.35}$                               & $\underline{38.28}$                               & $40.81$                             & $\mathbf{39.47}$                   & $\mathbf{22.50}$                  & $\mathbf{22.50}$                    & $\mathbf{28.91}$                   & $64.09$                           & $89.06$                             & $88.91$                            \\\hdashline[0.5pt/1pt]
			\hdashline[0.5pt/3pt]\rule{0pt}{10pt}MLP &              & \multicolumn{3}{c}{{$84.11$}}                        & \multicolumn{3}{c}{{$52.49$}}                    & \multicolumn{3}{c}{{$32.80$}}                     & \multicolumn{3}{c}{{$70.69$}}                                                                                                                                                                                                                                                                                                                              \\ \bottomrule
			\multicolumn{14}{l}{$^\downarrow$The lower number indicates better attack performance. $^\dagger$Runs with SeqGIA framework.  }                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\
		\end{tabular}}
\end{table}
\textbf{Evaluation protocol.}
We use a $3$-layer GCN as the surrogate model to generate perturbed graphs with various GIA attacks, and report the mean accuracy of defenses from multiple runs.
Details are in Appendix~\ref{sec:model_setting_appdx}.
For in-detail analysis of attack performance, we categorize all defenses into three folds by their robustness: Vanilla, \textbf{Robust}, and Extreme Robust (\textbf{Combo}) (Table~\ref{tab:defense_category}).
To examine how much an attack satisfies the homophily unnoticeability and its upper limits, we report \textit{maximum test accuracy} of both homophily defenders (\textbf{Homo}) and defenses from the last two categories.


\subsection{Empirical Performance}
In Table~\ref{tab:eval_non_targeted} and Table~\ref{tab:eval_targeted}, we report the non-targeted and targeted attack performance of various GIA methods, respectively.
We bold out the best attack and underline the second-best attack when combating against defenses from each category.
Full results are in Appendix~\ref{sec:eval_nontarget_detailed} and Appendix~\ref{sec:eval_target_detailed}.

\textbf{Performance of non-targeted attacks.}
In Table~\ref{tab:eval_non_targeted}, we can see that HAO significantly improves the performance of \textit{all} attacks on \textit{all} datasets up to $30\%$, which implies the effectiveness and versatility of HAO.
Especially, even coupled with a random injection strategy (PGD), HAO can attack robust models to be comparable with or inferior to simple MLP which does not consider relational information.
Meanwhile, adaptive injection strategies outperform previous methods PGD and TDGIA by a non-trivial margin for most cases, which further indicates that they are more suitable for HAO.


\textbf{Performance of targeted attack on large-scale graphs.}
In Table~\ref{tab:eval_targeted}, HAO also improves the targeted attack performance of \textit{all} attack methods on \textit{all} datasets by a significant margin of up to $15\%$,
which implies that the benefits of incorporating HAO are universal. Besides, adaptive injections can further improve the performance of attacks and establish the new state-of-the-art coupled with HAO.


\subsection{Analysis and Discussions}

\begin{figure}[t]
	\topspace
	\begin{subfigure}[c]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/cora_weights.pdf}
		\caption{Varying $\lambda$ in HAO}
		\label{fig:ablation_hao_coe}
	\end{subfigure}
	\hfill
	\begin{subfigure}[c]{0.64\textwidth}
		\scriptsize
		\centering\resizebox{0.95\textwidth}{!}{
			\begin{tabular}{lcccccc}
				\toprule
				\textbf{Model} & \textbf{Cora}$^\dagger$ & \textbf{Computers}$^\dagger$ & \textbf{Arxiv}$^\dagger$ & \textbf{Computers}$^\ddagger$ & \textbf{Aminer}$^\ddagger$ & \textbf{Reddit}$^\ddagger$ \\\midrule
				Clean          & $84.74$                 & $92.25$                      & $70.44$                  & $91.68$                       & $62.39$                    & $95.51$                    \\
				PGD            & $61.09$                 & $61.75$                      & $54.23$                  & $62.41$                       & $26.13$                    & $62.72$                    \\
				\hfill +HAO    & $\underline{56.63}$     & $\underline{59.16}$          & $\underline{45.05}$      & $59.09$                       & $\underline{22.15}$        & $56.99$                    \\
				MetaGIA        & $60.56$                 & $61.75$                      & $53.69$                  & $62.08$                       & $32.78$                    & $60.14$                    \\
				\hfill +HAO    & $58.51$                 & $60.29$                      & $48.48$                  & $\underline{58.63}$           & $29.91$                    & $\mathbf{54.14}$           \\
				AGIA           & $60.10$                 & $60.66$                      & $48.86$                  & $61.98$                       & $31.06$                    & $59.96$                    \\
				\hfill +HAO    & $\mathbf{53.79}$        & $\mathbf{58.71}$             & $48.86$                  & $\mathbf{58.37}$              & $26.51$                    & $56.36$                    \\
				TDGIA          & $66.86$                 & $66.79$                      & $49.73$                  & $62.47$                       & $32.37$                    & $57.97$                    \\
				\hfill +HAO    & $65.22$                 & $65.46$                      & $49.54$                  & $59.67$                       & $22.32$                    & $\underline{54.32}$        \\
				ATDGIA         & $61.14$                 & $65.07$                      & $46.53$                  & $64.66$                       & $24.72$                    & $61.25$                    \\
				\hfill +HAO    & $58.13$                 & $63.31$                      & $\mathbf{44.40}$         & $59.27$                       & $\mathbf{17.62}$           & $56.90$                    \\\bottomrule
				\multicolumn{7}{l}{The lower is better. $^\dagger$Non-targeted attack. $^\ddagger$Targeted attack.  }
			\end{tabular}}
		\caption{Averaged performance across all defense models}
		\label{tab:averaged_performance}
	\end{subfigure}
	\caption{(a): Effects of HAO with different weights; (b) Averaged attack performance of various attacks with or without HAO against both homophily defenders and other defense models. }
\end{figure}

\begin{figure}[t]
	\centering
	\hfill
	\begin{subfigure}[b]{0.322\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/grb-cora_node_sims_atk_tdgia.pdf}
		\caption{Homophily change}
		\label{fig:gia_homophily_dist_node_atk_hao}
	\end{subfigure}
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/cora_budget_tdgia.pdf}
		\caption{Varying node budgets}
		\label{fig:ablation_node_budgets}
	\end{subfigure}
	\begin{subfigure}[b]{0.319\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/cora_edge_budget_tdgia.pdf}
		\caption{Varying edge budgets}
		\label{fig:ablation_edge_budgets}
	\end{subfigure}
	\caption{(a) Homophily changes after attacked by GIA without HAO (orange) and GIA with HAO (canny); (b), (c) Attack performance against GCN and EGuard with different node and edge budgets. $\bullet$ indicates attack with defenses and $\blacktriangle$ indicates attack without defenses;}
	\label{fig:abalation_attacked_graph}
\end{figure}

\textbf{Effects of HAO.} Though HAO can substantially improve GIA methods under defenses, we find it essentially trades with the performance under no defenses.
In Fig.~\ref{fig:ablation_hao_coe}, as the weight for regularization term $\lambda$ increases, HAO trades slightly more of the performance against GCN for the performance against homophily defenders.
Finally, GIA reduces the performance of both GNNs with defenses and without defenses to be inferior to MLP.
Additionally, as also shown in Table~\ref{tab:averaged_performance}, the trade-off will not hurt the overall performance while consistently brings benefits up to $5\%$.



\textbf{Analysis of the perturbed graphs.}
In Fig.~\ref{fig:gia_homophily_dist_node_atk_hao}, we also analyze the homophily distribution changes after the attack. It turns out that GIA with HAO can effectively preserve the homophily while still conducting effective attacks.
Similar analysis on other datasets can be found in Appendix~\ref{sec:homophily_appdx}.

\textbf{Attacks with limited budgets.}
We also examine the performance of GIA methods with or without HAO varying different node and edge budgets.
Fig.~\ref{fig:ablation_node_budgets} and Fig.~\ref{fig:ablation_edge_budgets} show that HAO can consistently improve the overall performance by slightly trading with the performance under no defenses.




==> GIA-HAO/6_conclusion.tex <==

\section{Conclusions}
In this paper, we explored the advantages and limitations of GIA by comparing it with GMA.
Though we found that GIA can be provably more harmful than GMA,
the severe damage to the homophily makes it easily defendable by homophily defenders.
Hence we introduced homophily unnoticeability for GIA to constrain the damage and proposed HAO to instantiate it.
Extensive experiments show that GIA with HAO can break homophily defenders and substantially outperform all previous works.
We provide more discussions and future directions based on HAO in Appendix~\ref{sec:discussion_future_appdx}.


==> GIA-HAO/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

